Face Identity Disentanglement via Latent Space Mapping

Learning disentangled representations of data is a fundamental problem in artificial intelligence. Specifically, disentangled latent representations allow generative models to control and compose the disentangled factors in the synthesis process. Current methods, however, require extensive supervision and training, or instead, noticeably compromise quality. In this paper, we present a method that learns how to represent data in a disentangled way, with minimal supervision, manifested solely using available pre-trained networks. Our key insight is to decouple the processes of disentanglement and synthesis, by employing a leading pre-trained unconditional image generator, such as StyleGAN. By learning to map into its latent space, we leverage both its state-of-the-art quality, and its rich and expressive latent space, without the burden of training it. We demonstrate our approach on the complex and high dimensional domain of human heads. We evaluate our method qualitatively and quantitatively, and exhibit its success with de-identification operations and with temporal identity coherency in image sequences. Through extensive experimentation, we show that our method successfully disentangles identity from other facial attributes, surpassing existing methods, even though they require more training and supervision.

==> ablation.tex <==
\section{ablation}
\label{sec:ablation}

In the following we present an ablation study that analyzes the contribution of individual components and losses in our proposed method. 
One of the most intriguing components of our method is $D_{\mathcal{W}}$, which encourages the mapping network to predict latent representations that lie within StyleGAN's $\mathcal{W}$ space. To validate its affect, we train a baseline model,  \yn{\st{the} that} consists of our architecture without the discriminator $D_{\mathcal{W}}$ and its associated adversarial losses.
We explore and compare three different $\mathcal{W}$ spaces: (i) StyleGAN's original, ours and the baseline predicted spaces. We sample 10$K$ vectors from each space and compute PCA, visualized in \figref{fig:ablation_W_PCA}. As can be clearly seen, our predicted $\mathcal{W}$ coincides with StyleGAN's $\mathcal{W}$, while the baseline's $\mathcal{W}$ is significantly different, indicating that $D_{\mathcal{W}}$ is crucial for mapping $z$ into the actual $\mathcal{W}$ space of the pre-trained generator.
Furthermore, as stated by Karras et al. \shortcite{karras2019style, karras2019analyzing}, large \ync{they are not large, they are "extreme" in the sense that they lie far away from most of the data. StyleGAN original paper uses the term "extreme" to define this motion } regions in the latent space often correspond to generated images with inferior quality and resemblance to the real data distribution. Without $D_{\mathcal{W}}$, the predictions may lie in peripheral regions of $\mathcal{W}$, causing the generation of erroneous images, \yn{such as those in} \figref{fig:compare_ablation_images}.

\begin{figure}
	\centering
	\includegraphics[width=\linewidth]{figures/ablation_W_PCA}
	\caption{Dimension reduction of different configurations of $\mathcal{W}$, using PCA (n=2). As can be clearly seen, our predicted $\mathcal{W}$ space coincides with StyleGAN's, expanding it only slightly. However, without $D_{\mathcal{W}}$ the predicted $\mathcal{W}$ space is significantly different, stressing the necessity of $D_{\mathcal{W}}$. }
	\label{fig:ablation_W_PCA}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/ablation_compare.pdf}
    \caption{The effect of $D_\mathcal{W}$. Images in the top row were generated by our baseline without $D_\mathcal{W}$, images in the bottom row were generated using our method on the same inputs.}
    \label{fig:compare_ablation_images}
\end{figure}


Next, we evaluate the contribution of our landmarks consistency loss. This loss is calculated using an accessible off-the-shelf network, pre-trained on an independent dataset and task. In the following, we train our network without $E_{lnd}$, forming a baseline, and show that the supervision of the landmarks network serves merely to improve the attributes preservation, but is not required for disentanglement.
%
Quantitative evaluation is presented in \tabref{tab:quantitative_ablation}. As can be seen, removing $E_{lnd}$ decreases only the expression and pose preservation. Yet, even with this decrease the baseline is overall superior to LORD in those aspects.
Note that, since this landmarks supervision is not necessary to perform the disentanglement, our overall supervision is significantly weaker than the common class-supervision used by other methods. 

\begin{table*}
    \begin{center}
        \begin{tabular}{l c c c c}
        \toprule
         \multicolumn{1}{c}{Method}  &  \small{FID}  $\downarrow$ & \small{Identity}  $\uparrow$ & \small{Expression}   $\downarrow$ & \small{Pose}  $\downarrow$ \\
        \midrule
        \small{LORD \cite{gabbay2019demystifying}} & 23.08 & 0.20 $\pm$ 0.11 & 0.085 $\pm$ 0.018 & 13.34 $\pm$ 15.00  \\
        \small{Ours w/o $\mathcal{L}_{lnd}$} & 6.45 & \textbf{0.63 $\pm$ 0.08} & 0.023 $\pm$ 0.017 & 13.90 $\pm$ 13.36  \\
        \small{Ours} & \textbf{4.28} & 0.60 $\pm$ 0.09 & \textbf{0.017 $\pm$ 0.019} & \textbf{9.74 $\pm$ 13.16} \\
        \bottomrule
        \end{tabular}
    \end{center}
    \caption{Quantitative ablation}
    \label{tab:quantitative_ablation}
\end{table*}

